Pagination: It's what you say, not how long it takes to say it

Pagination - the process of determining where to break an article across pages in a multi-article layout is a common layout challenge for most commercially printed newspapers and magazines. To date, no one has created an algorithm that determines a minimal pagination break point based on the content of the article. Existing approaches for automatic multi-article layout focus exclusively on maximizing content (number of articles) and optimizing aesthetic presentation (e.g., spacing between articles). However, disregarding the semantic information within the article can lead to overly aggressive cutting, thereby eliminating key content and potentially confusing the reader, or setting too generous of a break point, thereby leaving in superfluous content and making automatic layout more difficult. This is one of the remaining challenges on the path from manual layouts to fully automated processes that still ensure article content quality. In this work, we present a new approach to calculating a document minimal break point for the task of pagination. Our approach uses a statistical language model to predict minimal break points based on the semantic content of an article. We then compare 4 novel candidate approaches, and 4 baselines (currently in use by layout algorithms). Results from this experiment show that one of our approaches strongly outperforms the baselines and alternatives. Results from a second study suggest that humans are not able to agree on a single "best" break point. Therefore, this work shows that a semantic-based lower bound break point prediction is necessary for ideal automated document synthesis within a real-world context.

==> compareMethodsAll_hist.tex <==
\begin{table}
 \centering
{\tiny 
	\rowcolors{2}{white}{tableShade}
	\begin{supertabular}{c l c c c}
	& {\bf Algorithm} & {\bf Mean (sd)} & {\bf Median} & {\bf Histogram} \\\midrule

\cellcolor{white}	&	\sOne	&	2.12 (1.08)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.82 \sparkspike 0.25 0.57 \sparkspike 0.38 0.46 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.29 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.01 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.83 (1.32)	&	3.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.43 \sparkspike 0.25 0.47 \sparkspike 0.38 0.58 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.37 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.31 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.78 (1.41)	&	3.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.48 \sparkspike 0.25 0.51 \sparkspike 0.38 0.45 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.57 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.08 \sparkspike 0.75 0.00 \sparkspike 0.88 0.06  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.33 (1.23)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.02 \sparkspike 0.38 0.20 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.27 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.62 \sparkspike 0.75 0.64 \sparkspike 0.88 0.40  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.70 (1.11)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.16 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.08 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.43 \sparkspike 0.75 1.00 \sparkspike 0.88 0.47  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.61 (1.17)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.04 \sparkspike 0.38 0.15 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.07 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.53 \sparkspike 0.75 0.92 \sparkspike 0.88 0.45  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.99 (1.81)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.04 \sparkspike 0.25 0.25 \sparkspike 0.38 0.25 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.17 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.52 \sparkspike 0.75 0.27 \sparkspike 0.88 0.65  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf Buisness}\end{sideways}}	&	\kc	&	4.47 (1.64)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.04 \sparkspike 0.25 0.34 \sparkspike 0.38 0.22 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.35 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.67 \sparkspike 0.75 0.24 \sparkspike 0.88 0.29  \end{sparkline}	 \\
\hline\hline
\cellcolor{white}	&	\sOne	&	1.43 (0.72)	&	1.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 1.00 \sparkspike 0.25 0.35 \sparkspike 0.38 0.09 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.04 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.00 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.08 (0.92)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.40 \sparkspike 0.25 0.71 \sparkspike 0.38 0.26 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.07 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.04 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.24 (1.05)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.40 \sparkspike 0.25 0.54 \sparkspike 0.38 0.32 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.18 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.03 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.23 (1.10)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.10 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.19 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.54 \sparkspike 0.75 0.46 \sparkspike 0.88 0.16  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.88 (1.03)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.00 \sparkspike 0.38 0.04 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.06 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.32 \sparkspike 0.75 0.61 \sparkspike 0.88 0.43  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.42 (1.05)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.10 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.10 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.49 \sparkspike 0.75 0.60 \sparkspike 0.88 0.18  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.70 (1.78)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.03 \sparkspike 0.25 0.14 \sparkspike 0.38 0.32 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.17 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.28 \sparkspike 0.75 0.18 \sparkspike 0.88 0.35  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf Entertainment}\end{sideways}}	&	\kc	&	3.82 (1.62)	&	3.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.05 \sparkspike 0.25 0.27 \sparkspike 0.38 0.45 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.20 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.24 \sparkspike 0.75 0.13 \sparkspike 0.88 0.12  \end{sparkline}	 \\
\hline\hline
\cellcolor{white}	&	\sOne	&	1.72 (0.93)	&	1.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.91 \sparkspike 0.25 0.50 \sparkspike 0.38 0.16 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.13 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.00 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.43 (1.17)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.39 \sparkspike 0.25 0.59 \sparkspike 0.38 0.44 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.14 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.13 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.40 (1.31)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.52 \sparkspike 0.25 0.50 \sparkspike 0.38 0.28 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.29 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.08 \sparkspike 0.75 0.00 \sparkspike 0.88 0.02  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.30 (0.91)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.00 \sparkspike 0.38 0.10 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.11 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.77 \sparkspike 0.75 0.61 \sparkspike 0.88 0.11  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.89 (0.81)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.00 \sparkspike 0.38 0.03 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.05 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.30 \sparkspike 0.75 1.00 \sparkspike 0.88 0.31  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.65 (0.94)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.08 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.05 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.46 \sparkspike 0.75 0.87 \sparkspike 0.88 0.23  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.79 (1.62)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.13 \sparkspike 0.38 0.31 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.24 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.41 \sparkspike 0.75 0.23 \sparkspike 0.88 0.36  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf Politics}\end{sideways}}	&	\kc	&	4.37 (1.48)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.21 \sparkspike 0.38 0.29 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.33 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.53 \sparkspike 0.75 0.15 \sparkspike 0.88 0.18  \end{sparkline}	 \\
\hline\hline
\cellcolor{white}	&	\sOne	&	1.62 (0.86)	&	1.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 1.00 \sparkspike 0.25 0.43 \sparkspike 0.38 0.21 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.08 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.00 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.42 (1.06)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.32 \sparkspike 0.25 0.69 \sparkspike 0.38 0.40 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.22 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.07 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.44 (1.40)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.50 \sparkspike 0.25 0.57 \sparkspike 0.38 0.24 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.30 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.03 \sparkspike 0.75 0.03 \sparkspike 0.88 0.03  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.40 (1.17)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.00 \sparkspike 0.38 0.12 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.26 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.46 \sparkspike 0.75 0.53 \sparkspike 0.88 0.33  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	6.12 (1.02)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.00 \sparkspike 0.38 0.04 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.08 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.30 \sparkspike 0.75 0.50 \sparkspike 0.88 0.79  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.81 (1.10)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.00 \sparkspike 0.38 0.08 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.10 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.46 \sparkspike 0.75 0.50 \sparkspike 0.88 0.57  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.52 (1.65)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.03 \sparkspike 0.25 0.14 \sparkspike 0.38 0.39 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.33 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.33 \sparkspike 0.75 0.16 \sparkspike 0.88 0.32  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf Sports}\end{sideways}}	&	\kc	&	4.40 (1.59)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.16 \sparkspike 0.38 0.45 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.30 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.35 \sparkspike 0.75 0.17 \sparkspike 0.88 0.26  \end{sparkline}	 \\
\hline\hline
\cellcolor{white}	&	\sOne	&	1.82 (0.99)	&	1.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 1.00 \sparkspike 0.25 0.40 \sparkspike 0.38 0.38 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.13 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.00 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.50 (1.31)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.58 \sparkspike 0.25 0.46 \sparkspike 0.38 0.38 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.36 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.13 \sparkspike 0.75 0.01 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.47 (1.27)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.61 \sparkspike 0.25 0.41 \sparkspike 0.38 0.38 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.43 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.09 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.13 (1.33)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.06 \sparkspike 0.38 0.18 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.35 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.41 \sparkspike 0.75 0.65 \sparkspike 0.88 0.26  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.78 (1.32)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.03 \sparkspike 0.38 0.13 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.16 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.35 \sparkspike 0.75 0.49 \sparkspike 0.88 0.76  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.27 (1.42)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.06 \sparkspike 0.38 0.28 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.11 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.42 \sparkspike 0.75 0.70 \sparkspike 0.88 0.35  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.58 (1.89)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.08 \sparkspike 0.25 0.31 \sparkspike 0.38 0.28 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.13 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.43 \sparkspike 0.75 0.28 \sparkspike 0.88 0.41  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf Technology}\end{sideways}}	&	\kc	&	4.10 (1.83)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.13 \sparkspike 0.25 0.35 \sparkspike 0.38 0.29 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.31 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.38 \sparkspike 0.75 0.19 \sparkspike 0.88 0.27  \end{sparkline}	 \\
\hline\hline
\cellcolor{white}	&	\sOne	&	1.74 (0.94)	&	1.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 1.00 \sparkspike 0.25 0.53 \sparkspike 0.38 0.21 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.15 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.00 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.39 (1.13)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.42 \sparkspike 0.25 0.75 \sparkspike 0.38 0.42 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.18 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.13 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.27 (1.27)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.65 \sparkspike 0.25 0.59 \sparkspike 0.38 0.28 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.26 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.09 \sparkspike 0.75 0.01 \sparkspike 0.88 0.01  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.05 (1.17)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.02 \sparkspike 0.38 0.17 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.42 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.56 \sparkspike 0.75 0.52 \sparkspike 0.88 0.19  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.79 (1.15)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.09 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.16 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.39 \sparkspike 0.75 0.64 \sparkspike 0.88 0.61  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.50 (1.19)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.17 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.15 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.51 \sparkspike 0.75 0.67 \sparkspike 0.88 0.39  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.46 (1.81)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.05 \sparkspike 0.25 0.21 \sparkspike 0.38 0.48 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.26 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.28 \sparkspike 0.75 0.20 \sparkspike 0.88 0.41  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf US News}\end{sideways}}	&	\kc	&	3.90 (1.61)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.08 \sparkspike 0.25 0.32 \sparkspike 0.38 0.50 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.30 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.32 \sparkspike 0.75 0.24 \sparkspike 0.88 0.13  \end{sparkline}	 \\
\hline\hline
\cellcolor{white}	&	\sOne	&	2.02 (1.07)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 1.00 \sparkspike 0.25 0.72 \sparkspike 0.38 0.40 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.29 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.02 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.64 (1.17)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.40 \sparkspike 0.25 0.90 \sparkspike 0.38 0.46 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.52 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.15 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.49 (1.24)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.65 \sparkspike 0.25 0.72 \sparkspike 0.38 0.40 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.57 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.09 \sparkspike 0.75 0.01 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	4.88 (1.33)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.04 \sparkspike 0.25 0.06 \sparkspike 0.38 0.32 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.40 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.77 \sparkspike 0.75 0.62 \sparkspike 0.88 0.23  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.66 (1.39)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.05 \sparkspike 0.38 0.21 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.18 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.44 \sparkspike 0.75 0.68 \sparkspike 0.88 0.87  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.37 (1.32)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.04 \sparkspike 0.38 0.26 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.33 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.46 \sparkspike 0.75 0.85 \sparkspike 0.88 0.50  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.55 (1.71)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.06 \sparkspike 0.25 0.26 \sparkspike 0.38 0.46 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.33 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.62 \sparkspike 0.75 0.24 \sparkspike 0.88 0.46  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways} \cellcolor{white} {\bf World News}\end{sideways}}	&	\kc	&	4.20 (1.67)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth \smallSparklineWidth\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.10 \sparkspike 0.25 0.32 \sparkspike 0.38 0.52 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.39 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.57 \sparkspike 0.75 0.24 \sparkspike 0.88 0.29  \end{sparkline}	 \\

	
	\end{supertabular}

\caption{Performance Per Subject}{{\scriptsize{\em  \sparklineFootnote}}} 
\label{tab:compareBySubject}
}
\end{table}

==> compareMethods_hist.tex <==
\begin{table}
 \centering 
	\rowcolors{2}{white}{tableShade}
	\begin{supertabular}{c l c c c}
	& {\bf Algorithm} & {\bf Mean (sd)} & {\bf Median} & {\bf Histogram} \\\toprule
\cellcolor{white}	&	\sOne	&	1.78 (0.97)	&	1.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 1.00 \sparkspike 0.25 0.50 \sparkspike 0.38 0.27 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.15 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.00 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\sTwo	&	2.47 (1.18)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.43 \sparkspike 0.25 0.67 \sparkspike 0.38 0.43 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.26 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.13 \sparkspike 0.75 0.00 \sparkspike 0.88 0.00  \end{sparkline}	 \\
\cellcolor{white}	&	\pOne	&	2.44 (1.29)	&	2.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.55 \sparkspike 0.25 0.57 \sparkspike 0.38 0.34 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.37 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.07 \sparkspike 0.75 0.01 \sparkspike 0.88 0.02  \end{sparkline}	 \\
\cellcolor{white}	&	\tw	&	5.19 (1.20)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.01 \sparkspike 0.25 0.02 \sparkspike 0.38 0.17 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.29 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.61 \sparkspike 0.75 0.59 \sparkspike 0.88 0.24  \end{sparkline}	 \\
\cellcolor{white}	&	\na	&	5.83 (1.14)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.01 \sparkspike 0.38 0.10 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.11 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.37 \sparkspike 0.75 0.73 \sparkspike 0.88 0.61  \end{sparkline}	 \\
\cellcolor{white}	&	\nc	&	5.52 (1.19)	&	6.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.00 \sparkspike 0.25 0.02 \sparkspike 0.38 0.16 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.12 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.50 \sparkspike 0.75 0.74 \sparkspike 0.88 0.38  \end{sparkline}	 \\
\cellcolor{white}	&	\ka	&	4.66 (1.76)	&	5.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.04 \sparkspike 0.25 0.21 \sparkspike 0.38 0.37 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.24 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.41 \sparkspike 0.75 0.23 \sparkspike 0.88 0.43  \end{sparkline}	 \\
\multirow{-8}{*}[-0.1em]{\begin{sideways}{\small \cellcolor{white} {\bf All Subject Areas}}\end{sideways}}	&	\kc	&	4.18 (1.65)	&	4.00	&	 \begin{sparkline}{7} \sparkspikewidth 1.05mm\definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.12 0.06 \sparkspike 0.25 0.29 \sparkspike 0.38 0.41 \definecolor{sparkspikecolor}{gray}{0.0}\sparkspike 0.50 0.31 \definecolor{sparkspikecolor}{gray}{\sparkGray}\sparkspike 0.62 0.44 \sparkspike 0.75 0.20 \sparkspike 0.88 0.22  \end{sparkline}	 \\

	
	\end{supertabular}

\caption{Overall Performance}{{\scriptsize{\em \sparklineFootnote  }}} 
\label{tab:compareOverall}
\end{table}

==> data/SLM_article.tex <==
\begin{figure}
 \centering
 \pgfplotsset{width=2.7in}
\begin{tikzpicture}
	\begin{axis}[
			xlabel={Everything Up To X\% of Document}, 	xtick pos=left, 
			ytick pos=left,		ylabel={Cumulative \% of Ratings},	%ymax = .5,
			y tick label style={/pgf/number format/.cd, fixed, fixed zerofill, precision=0, /tikz/.cd},
			xticklabels/.append style={font=\smlFontSize},
			every axis/.append style={font=\smlFontSize},
			legend pos=outer north east,
			axis lines=left,
			extra x ticks = 20, 	extra x tick labels = ,		extra x tick style  = { grid = major, \slmLineColor },
		]
		\addplot [no markers, black ,mark size=\markSize] table [col sep=comma,x=lookup, y=TooShort] {data/SLM_article.csv};
		\addplot [no markers, black ,dashed] table [col sep=comma,x=lookup, y=Ideal] {data/SLM_article.csv};
		\addplot [no markers, black , thick] table [col sep=comma,x=lookup, y=TooLong] {data/SLM_article.csv};
		\legend{Too Short,Ideal, Too Long}
	\end{axis}
\end{tikzpicture} 
  \caption{When Failure Occurs}{{\em {\scriptsize Additional Text}}}\label{fig:failure}
\end{figure}

==> section_layout.tex <==
\section{Layout Performance Improvements}

The above study focused exclusively on the objective rating of a breakpoint in terms of article semantic content. The outcome showed that the SLM approach was the most ``balanced'' break point between length and semantic content. In addition, these results suggested that because SLM was more aggressive than Twenty Percent, it would provide a greater degree of flexibility to the automatic layout algorithm (by requiring less text as a minimal break point when possible). 

We illustrate the increased flexibility the SLM approach provides, we within the context of a content clipping framework within an automated publishing system similar to \cite{Ahmadullin:2013dj} currently in use at \hp. This automated publishing system uses an XML structure to encode text blocks, figures, and their logical relationships. The results from the clip point analysis are used to set a binary attribute on paragraphs indicating whether a clip is allowed or not at that paragraph. Based on this, the layout algorithm is able to automatically choose from allowed clip points to trim articles as needed in order to improve the layout quality (defined in the following subsection \ref{sec:layoutMetric}). 

We directly compare the performance of SLM Article\footnote{SLM Article was used over SLM-Corpus because the automated publishing system does not aggregate multiple articles about the same topic into a corpus. Thus, we could not use the higher performing SLM Corpus approach in this context.} minimal breakpoint algorithm to that of the content agnostic Twenty Percent measure (tested above) which is currently in use at \hp within this system.  While not a comprehensive study, we perform one layout across each of our seven subject areas. Each layout consists of 8 articles from the same subject area (and same day of news).

%The input to our news layout engine is an XML file. The XML structure is composed of text blocks and figures.
%We encode content types and logical relationships as XML attributes. The results from the clip point analysis are used to set a binary attribute  on paragraphs indicating whether a clip is allowed or not at that paragraph.
%The layout algorithm is able to automatically choose from allowed clip points to trim articles as needed in order to improve the layout quality. We compare layouts using a content agnostic rule (retain at least 20\% of the article) versus our content aware clip point analysis presenting in this paper. Comparative layout scores (normalized log probability) are shown in Fig.XX
 
 \subsection{Comparative Layout Metric}\label{sec:layoutMetric}
 
The composition algorithm is based on a model of document quality, the probabilistic document model (PDM) \cite{DameraVenkata:2011hv,Ahmadullin:2013dj}. PDM explicitly models the dependency between key design choices including pagination (what content should be placed on a page), choice of relative arrangements for page elements (what template to use for each page), and template parameters (physical dimensions of various page elements like images, whitespace etc.). The coupling between these design variables is explicitly modeled as a Bayesian network.
 
PDM is in fact a micro model for document quality that associates a probability (or log probability quality score) distribution with each conditional design choice made on each page. These probability distributions (e.g. whitespace, template, variance of acceptable whitespace) are specified at design time by a document designer (see  \cite{DameraVenkata:2011hv,Ahmadullin:2013dj} for details). Thus, if all factors are kept the same (content, parameters, etc) and we only alter the minimal pagination breakpoint, we can use the PDM rating of a document as a metric for how well the layout performed.
 

%it also suggested that its smaller minimal break point would provide increased flexibility to the automatic layout algorithm. In order to explicitly test this supposition, we integrated the SLM-Article\footnote{SLM Article was used over SLM-Corpus because \software does not aggregate multiple articles about the same topic into a corpus. Thus, we could not use the higher performing SLM Corpus approach in this context.} and into the existing \software used at \hp (which currently employs the Twenty Percent algorithm as a lower bound). This allows us to directly compare the layout impact (not breakpoint content impact) the SLM based approach to the current standard used using the \textcolor{red} {METRIC} metic for layout flexibility \textcolor{red} {[CITE]}.

%\subsection{Evaluation}

%We use an automated document composition algorithm to compose documents from  multiple articles. In order to compose documents, one must make aesthetic decisions on how to paginate content, how to arrange page elements (text, images, graphics, sidebars etc.) on each page, how much to crop/scale images, how to manage whitespace etc. These decision variables are not mutually exclusive, making the aesthetic graphic design of documents a hard problem often requiring an expert design professional.
 

\subsection{Results}

These are forthcoming.
